6G White Paper on Localization and Sensing

This white paper explores future localization and sensing opportunities for beyond 5G wireless communication systems by identifying key technology enablers and discussing their underlying challenges, implementation issues, and identifying potential solutions. In addition, we present exciting new opportunities for localization and sensing applications, which will disrupt traditional design principles and revolutionize the way we live, interact with our environment, and do business. Following the trend initiated in the 5G NR systems, 6G will continue to develop towards even higher frequency ranges, wider bandwidths, and massive antenna arrays. In turn, this will enable sensing solutions with very fine range, Doppler and angular resolutions, as well as localization to cm-level degree of accuracy. Moreover, new materials, device types, and reconfigurable surfaces will allow network operators to reshape and control the electromagnetic response of the environment. At the same time, machine learning and artificial intelligence will leverage the unprecedented availability of data and computing resources to tackle the biggest and hardest problems in wireless communication systems. 6G will be truly intelligent wireless systems that will not only provide ubiquitous communication but also empower high accuracy localization and high-resolution sensing services. They will become the catalyst for this revolution by bringing about a unique new set of features and service capabilities, where localization and sensing will coexist with communication, continuously sharing the available resources in time, frequency and space. This white paper concludes by highlighting foundational research challenges, as well as implications and opportunities related to privacy, security, and trust. Addressing these challenges will undoubtedly require an inter-disciplinary and concerted effort from the research community.

==> 6G White Paper expert group 12_ Localization and Sensing/6Gacronym.tex <==
\begin{acronym}[mmmmm]
	% \acro{IP}{Internet Protocol}
	\acro{3GPP}[$3$GPP]{$3 \text{rd}$ Generation Partnership Project}
	\acro{ABS}{Almost Blank Sub-frame}
	\acro{ADSL}{Asymmetric Digital Subscriber Line}
	\acro{AF}{Amplify-and-Forward}
	\acro{AI}{Artificial Intelligence}
	\acro{ALBA-R}{Adaptive Load-Balanced Algorithm Rainbow}
	\acro{ALBA}{Adaptive Load-Balanced Algorithm}
	\acro{ALOHA}[ALOHA]{}
	\acro{AOA}{Angle Of Arrival}
	\acro{APDL}{Average Packet Delivery Latency}
	\acro{AP}{Access Point}
	\acro{ASE}{Average Spectral Efficiency}
	\acro{BAP}{Blocked Access Protocol}
	\acro{BB}{Busy Burst}
	\acro{BC}{Broadcast Channel}
	\acro{BPP}{Binomial Point Process}
	\acro{BS}{Base Station}
	\acro{CAA}{Channel Access Algorithm}
	\acro{CAPEX}{Capital Expenditure}
	\acro{CAP}{Channel Access Protocol}
	\acro{CCDF}{Complementary Cumulative Distribution Function}
	\acro{CCI}{Co-Channel Interference}
	\acro{CDF}{Cumulative Distribution Function}
	\acro{CDMA}{Code Division Multiple Access}
	\acro{CDR}{Convex Lenses Decision Region}
	\acro{CF}{Characteristic Function}
	\acro{CGF}{Contention-based Geographic Forwarding}
	\acro{CM}{Coordination Mechanism}
	\acro{COMP}{Coordinated Multi-Point}
	\acro{CPICH}{Common Pilot Channel}
	\acro{CRA}{Conflict Resolution Algorithm}
	\acro{CRD}{Contention Resolution Delay}
	\acro{CRI}{Contention Resolution Interval}
	\acro{CRP}{Contention Resolution Protocol}
	\acro{CRS}{Cell-specific Reference Signal}
	\acro{CR}{Contention Resolution}
	\acro{CSI}{Channel State Information}
	\acro{CSMA/CA}{Carrier Sense Multiple Access with Collision Avoidance}
	\acro{CSMA/CD}{Carrier Sense Multiple Access with Collision Detection}
	\acro{CSMA}{Carrier Sense Multiple Access}
	\acro{CTM}{Capetanakis-Tsybakov-Mikhailov}
	\acro{CTS}{Clear To Send}
	\acro{D2D}{Device-To-Device}
	\acro{DAS}{Distributed Antenna System}
        \acro{DAG}{Directed Acyclic Graph}
        \acro{DCF}{Distributed Coordination Function}
	\acro{DER}{Dynamic Exclusion Region}
	\acro{DF}{Decode-and-Forward}
	\acro{DHCP}{Dynamic Host Configuration Protoco}
	\acro{DL}{Downlink}
	\acro{DOA}{Direction of Arrival}
	\acro{DSL}{Digital Subscriber Line}
	\acro{E2E}{End-to-End}
	\acro{EDM}{Euclidean Distance Matrix}
	\acro{eMBB}{enhanced Mobile BroadBand}
	\acro{ES}{Evaluation Scenario}
	\acro{FAP}{Femto Access Point}
	\acro{FBS}{Femto Base Station}
	\acro{FD}{Full-Duplex}
	\acro{FDD}{Frequency Division Duplexing}
	\acro{FDM}{Frequency Division Multiplexing}
	\acro{FDR}{Forwarding Decision Region}
	\acro{FFR}{Fractional Frequency Reuse}
	\acro{FG}{Frequency Group}
	\acro{FPP}{First Passage Percolation}
	\acro{FUE}{Femto User Equipment}
	\acro{FU}{Femtocell User}
	\acro{GF}{Geographic Forwarding}
	\acro{GLIDER}{Gradient Landmark-Based Distributed Routing}
	\acro{GPSR}{Greedy Perimeter Stateless Routing}
	\acro{GeRaF}{Geographic Random Forwarding}
	\acro{HC}{Hard Core}
	\acro{HD}{Half-Duplex}
	\acro{HDR}[HDR]{High Data Rate}
	\acro{HII}{High Interference Indicator}
	\acro{HNB}{Home Node B}
        \acro{HTS}{High throughput Satellites}
	\acro{HN}[HetNet]{Heteronegeous Network}
	\acro{HOS}{Higher Order Statistics}
	\acro{HUE}{Home User Equipment}
	\acro{ICIC}{Inter-Cell Interference Coordination}
	\acro{ICT}{Information and Communications Technology}
	\acro{IEEE}[IEEE]{}
	\acro{IMT}{International Mobile Telecommunications}
	\acro{IP}{Interference Profile}
	\acro{IPR}{Intellectual Property Right}
	\acro{IoT}{Internet of Things}
	\acro{ITU}{International Telecommunication Union}
        \acro{KDE}{Kernel Density Estimation}
	\acro{KPI}{Key Performance Indicators}
	\acro{LMU}{Location Measurement Unit}
	\acro{LN}{Log-Normal}
	\acro{LTE}{Long Term Evolution}
	\acro{LoS}{Line-of-Sight}
        \acro{M2M}[M$2$M]{Machine-to-Machine}
	\acro{MACA}{Multiple Access with Collision Avoidance}
	\acro{MAC}{Medium Access Control}
        \acro{MEC}{Multi-Access Edge Computing}
	\acro{MCMC}{Markov Chain Monte Carlo}
	\acro{MBS}{Macro Base Station}
	\acro{MEC}{Multi-Access Edge Computing}
	\acro{MT}{Mellin Transform}
	\acro{MTC}{Machine Type Communication}
	\acro{MGF}{Moment Generating Function}
	\acro{MIMO}{Multiple-Input Multiple-Output}
	\acro{mMTC}{massive Machine Type Communications}
	\acro{MPP}{Marked Point Process}
	\acroplural{MPP}[MPPs]{Marked Point Processes}
	\acro{MRC}{Maximum Ratio Combining}
	\acro{MS}{Mobile Station}
	\acro{MTC}{Machine Type Communication}
	\acro{MUE}{Macro User Equipment}
	\acro{MU}{Macrocell User}
	\acro{NB}{Node B}
	\acro{NLoS}{Non Line-of-Sight}
        \acro{NOMA}{Non-Orthogonal Multiple Access}
	\acro{NR}{New Radio}
	\acro{NRT}{Non Real Time}
	\acro{OFDMA}{Orthogonal Frequency Division Multiple Access}
	\acro{OOP}{Object Oriented Programming}
	\acro{OPEX}{Operating Expenditure}
	\acro{OP}{Outage Probability}
	\acro{OS}{Order Statistic}
	\acro{PBS}{Pico Base Station}
	\acro{PCI}{Physical Cell Indicator}
	\acro{PC}{Power Control}
	\acro{PDF}{Probability Density Function}
	\acro{PDSR}{Packet Delivery Success Ratio}
	\acro{PGF}{Probability Generating Function}
	\acro{PMF}{Probability Mass Function}
	\acro{PPP}{Poisson Point Process}
	\acroplural{PPP}[PPPs]{Poisson Point Processes}
	\acro{PP}{Point Process}
	\acro{PRM}{Poisson Random Measure}
	\acro{PSS}{Primary Synchronization Channel}
	\acro{QoS}{Quality of Service}
	\acro{RAS}{Random Access System}
	\acro{RAT}{Radio Access Technology}
	\acro{RA}{Random Access}
	\acro{RCA}{Random Channel Access}
	\acro{RD}[R$\&$D]{Research $\&$ Development}
	\acro{REB}{Range Expansion Bias}
	\acro{RE}{Range Expansion}
	\acro{RF}{Radio Frequency}
	\acro{RFF}{Radio Frequency Fingerprinting}
	\acro{RIBF}{Regularized Incomplete Beta Function}
	\acro{RMA}{Random Multiple-Access}
	\acro{RMSE}{Root Mean Square Error}
	\acro{RNTP}{Relative Narrowband Transmit Power}
	\acro{RN}{Relay Node}
	\acro{RRM}{Radio Resource Management}
	\acro{RSA}{Relay Selection Algorithm}
	\acro{RSC}{Reliable Service Composition}
	\acro{RSRP}{Reference Signal Received Power}
	\acro{RSSI}{Received Signal Strength Indicator}
	\acro{RSS}{Received Signal Strength}
	\acro{RS}{Relay Selection}
	\acro{RTS}{Request to Send}
	\acro{RT}{Real Time}
	\acro{RV}{Random Variable}
	\acro{SC}{Selection Combining}
	\acro{SDR}{Sectoral Decision Region}
	\acro{SF}{Sub-Frame}
	\acro{SG}{Stochastic Geometry}
	\acro{SI}{Self-Interference}
	\acro{SIC}{Successive Interference Cancellation}
	\acro{SINR}{Signal-to-Interference plus Noise Ratio}
	\acro{SIP}{system in package}
	\acro{SIR}{Signal-to-Interference Ratio}
	\acro{SLN}{Shifted Log-Normal}
	\acro{SMP}{Semi-Markov Process}
	\acroplural{SMP}[SMPs]{Semi-Markov Processes}	
	\acro{SM}{State Machine}
	\acro{SNR}{Signal to Noise Ratio}
	\acro{SON}{Self-Organizing Network}
	\acro{SPP}{Spatial Poisson Process}
	\acroplural{SPP}[SPPs]{Spatial Poisson Processes}
	\acro{SSS}{Secondary Synchronization Channel}
	\acro{STA}{Standard Tree Algorithm}
        \acro{SAT\(5\)G}{Satellite and Terrestrial Network for \(5\)G}
	\acro{TAS}{Transmit Antenna Selection}
	\acro{TCP}{Transmission Control Protocol}
	\acro{TC}{Transmission Capacity}
	\acro{TDD}{Time Division Duplexing}	
	\acro{TDMA}{Time Division Multiple Access}	
	\acro{TOA}{Time of Arrival}
	\acro{TS}{Terminal Station}
	\acro{TTI}{Transmission Time Interval}
	\acro{TTT}{Time To Trigger}
	\acro{UDM}{Unit Disk Model}
	\acro{UD}{Unit Disk}
	\acro{UE}{User Equipment}
	\acro{ULUTRANSIM}[UL UTRANSim]{R6 Uplink UTRAN Simulator}
	\acro{UL}{Uplink}
	\acro{UML}{Unified Modeling Language}
	\acro{UoI}{User of Interest}
	\acro{UMTS}{Universal Mobile Telecommunications System}
	\acro{URC}{Ultra Reliable Communication}
	\acro{URLLC}{Ultra Reliable Low Latency Communications}
	\acro{WCDMA}{Wideband Code Division Multiple Access}
	\acro{WSN}{Wireless Sensor Network}
	\acro{iid}[\textup{i.i.d.}]{independent and identically distributed}
\end{acronym}


==> 6Gacronym.tex <==
\begin{acronym}[mmmmm]
	% \acro{IP}{Internet Protocol}
	\acro{3GPP}[$3$GPP]{$3 \text{rd}$ Generation Partnership Project}
	\acro{ABS}{Almost Blank Sub-frame}
	\acro{ADSL}{Asymmetric Digital Subscriber Line}
	\acro{AF}{Amplify-and-Forward}
	\acro{AI}{Artificial Intelligence}
	\acro{ALBA-R}{Adaptive Load-Balanced Algorithm Rainbow}
	\acro{ALBA}{Adaptive Load-Balanced Algorithm}
	\acro{ALOHA}[ALOHA]{}
	\acro{AOA}{Angle Of Arrival}
	\acro{APDL}{Average Packet Delivery Latency}
	\acro{AP}{Access Point}
	\acro{ASE}{Average Spectral Efficiency}
	\acro{BAP}{Blocked Access Protocol}
	\acro{BB}{Busy Burst}
	\acro{BC}{Broadcast Channel}
	\acro{BPP}{Binomial Point Process}
	\acro{BS}{Base Station}
	\acro{CAA}{Channel Access Algorithm}
	\acro{CAPEX}{Capital Expenditure}
	\acro{CAP}{Channel Access Protocol}
	\acro{CCDF}{Complementary Cumulative Distribution Function}
	\acro{CCI}{Co-Channel Interference}
	\acro{CDF}{Cumulative Distribution Function}
	\acro{CDMA}{Code Division Multiple Access}
	\acro{CDR}{Convex Lenses Decision Region}
	\acro{CF}{Characteristic Function}
	\acro{CGF}{Contention-based Geographic Forwarding}
	\acro{CM}{Coordination Mechanism}
	\acro{COMP}{Coordinated Multi-Point}
	\acro{CPICH}{Common Pilot Channel}
	\acro{CRA}{Conflict Resolution Algorithm}
	\acro{CRD}{Contention Resolution Delay}
	\acro{CRI}{Contention Resolution Interval}
	\acro{CRP}{Contention Resolution Protocol}
	\acro{CRS}{Cell-specific Reference Signal}
	\acro{CR}{Contention Resolution}
	\acro{CSI}{Channel State Information}
	\acro{CSMA/CA}{Carrier Sense Multiple Access with Collision Avoidance}
	\acro{CSMA/CD}{Carrier Sense Multiple Access with Collision Detection}
	\acro{CSMA}{Carrier Sense Multiple Access}
	\acro{CTM}{Capetanakis-Tsybakov-Mikhailov}
	\acro{CTS}{Clear To Send}
	\acro{D2D}{Device-To-Device}
	\acro{DAS}{Distributed Antenna System}
        \acro{DAG}{Directed Acyclic Graph}
        \acro{DCF}{Distributed Coordination Function}
	\acro{DER}{Dynamic Exclusion Region}
	\acro{DF}{Decode-and-Forward}
	\acro{DHCP}{Dynamic Host Configuration Protoco}
	\acro{DL}{Downlink}
	\acro{DOA}{Direction of Arrival}
	\acro{DSL}{Digital Subscriber Line}
	\acro{E2E}{End-to-End}
	\acro{EDM}{Euclidean Distance Matrix}
	\acro{eMBB}{enhanced Mobile BroadBand}
	\acro{ES}{Evaluation Scenario}
	\acro{FAP}{Femto Access Point}
	\acro{FBS}{Femto Base Station}
	\acro{FD}{Full-Duplex}
	\acro{FDD}{Frequency Division Duplexing}
	\acro{FDM}{Frequency Division Multiplexing}
	\acro{FDR}{Forwarding Decision Region}
	\acro{FFR}{Fractional Frequency Reuse}
	\acro{FG}{Frequency Group}
	\acro{FPP}{First Passage Percolation}
	\acro{FUE}{Femto User Equipment}
	\acro{FU}{Femtocell User}
	\acro{GF}{Geographic Forwarding}
	\acro{GLIDER}{Gradient Landmark-Based Distributed Routing}
	\acro{GPSR}{Greedy Perimeter Stateless Routing}
	\acro{GeRaF}{Geographic Random Forwarding}
	\acro{HC}{Hard Core}
	\acro{HD}{Half-Duplex}
	\acro{HDR}[HDR]{High Data Rate}
	\acro{HII}{High Interference Indicator}
	\acro{HNB}{Home Node B}
        \acro{HTS}{High throughput Satellites}
	\acro{HN}[HetNet]{Heteronegeous Network}
	\acro{HOS}{Higher Order Statistics}
	\acro{HUE}{Home User Equipment}
	\acro{ICIC}{Inter-Cell Interference Coordination}
	\acro{ICT}{Information and Communications Technology}
	\acro{IEEE}[IEEE]{}
	\acro{IMT}{International Mobile Telecommunications}
	\acro{IP}{Interference Profile}
	\acro{IPR}{Intellectual Property Right}
	\acro{IoT}{Internet of Things}
	\acro{ITU}{International Telecommunication Union}
        \acro{KDE}{Kernel Density Estimation}
	\acro{KPI}{Key Performance Indicators}
	\acro{LMU}{Location Measurement Unit}
	\acro{LN}{Log-Normal}
	\acro{LTE}{Long Term Evolution}
	\acro{LoS}{Line-of-Sight}
        \acro{M2M}[M$2$M]{Machine-to-Machine}
	\acro{MACA}{Multiple Access with Collision Avoidance}
	\acro{MAC}{Medium Access Control}
        \acro{MEC}{Multi-Access Edge Computing}
	\acro{MCMC}{Markov Chain Monte Carlo}
	\acro{MBS}{Macro Base Station}
	\acro{MEC}{Multi-Access Edge Computing}
	\acro{MT}{Mellin Transform}
	\acro{MTC}{Machine Type Communication}
	\acro{MGF}{Moment Generating Function}
	\acro{MIMO}{Multiple-Input Multiple-Output}
	\acro{mMTC}{massive Machine Type Communications}
	\acro{MPP}{Marked Point Process}
	\acroplural{MPP}[MPPs]{Marked Point Processes}
	\acro{MRC}{Maximum Ratio Combining}
	\acro{MS}{Mobile Station}
	\acro{MTC}{Machine Type Communication}
	\acro{MUE}{Macro User Equipment}
	\acro{MU}{Macrocell User}
	\acro{NB}{Node B}
	\acro{NLoS}{Non Line-of-Sight}
        \acro{NOMA}{Non-Orthogonal Multiple Access}
	\acro{NR}{New Radio}
	\acro{NRT}{Non Real Time}
	\acro{OFDMA}{Orthogonal Frequency Division Multiple Access}
	\acro{OOP}{Object Oriented Programming}
	\acro{OPEX}{Operating Expenditure}
	\acro{OP}{Outage Probability}
	\acro{OS}{Order Statistic}
	\acro{PBS}{Pico Base Station}
	\acro{PCI}{Physical Cell Indicator}
	\acro{PC}{Power Control}
	\acro{PDF}{Probability Density Function}
	\acro{PDSR}{Packet Delivery Success Ratio}
	\acro{PGF}{Probability Generating Function}
	\acro{PMF}{Probability Mass Function}
	\acro{PPP}{Poisson Point Process}
	\acroplural{PPP}[PPPs]{Poisson Point Processes}
	\acro{PP}{Point Process}
	\acro{PRM}{Poisson Random Measure}
	\acro{PSS}{Primary Synchronization Channel}
	\acro{QoS}{Quality of Service}
	\acro{RAS}{Random Access System}
	\acro{RAT}{Radio Access Technology}
	\acro{RA}{Random Access}
	\acro{RCA}{Random Channel Access}
	\acro{RD}[R$\&$D]{Research $\&$ Development}
	\acro{REB}{Range Expansion Bias}
	\acro{RE}{Range Expansion}
	\acro{RF}{Radio Frequency}
	\acro{RFF}{Radio Frequency Fingerprinting}
	\acro{RIBF}{Regularized Incomplete Beta Function}
	\acro{RMA}{Random Multiple-Access}
	\acro{RMSE}{Root Mean Square Error}
	\acro{RNTP}{Relative Narrowband Transmit Power}
	\acro{RN}{Relay Node}
	\acro{RRM}{Radio Resource Management}
	\acro{RSA}{Relay Selection Algorithm}
	\acro{RSC}{Reliable Service Composition}
	\acro{RSRP}{Reference Signal Received Power}
	\acro{RSSI}{Received Signal Strength Indicator}
	\acro{RSS}{Received Signal Strength}
	\acro{RS}{Relay Selection}
	\acro{RTS}{Request to Send}
	\acro{RT}{Real Time}
	\acro{RV}{Random Variable}
	\acro{SC}{Selection Combining}
	\acro{SDR}{Sectoral Decision Region}
	\acro{SF}{Sub-Frame}
	\acro{SG}{Stochastic Geometry}
	\acro{SI}{Self-Interference}
	\acro{SIC}{Successive Interference Cancellation}
	\acro{SINR}{Signal-to-Interference plus Noise Ratio}
	\acro{SIP}{system in package}
	\acro{SIR}{Signal-to-Interference Ratio}
	\acro{SLN}{Shifted Log-Normal}
	\acro{SMP}{Semi-Markov Process}
	\acroplural{SMP}[SMPs]{Semi-Markov Processes}	
	\acro{SM}{State Machine}
	\acro{SNR}{Signal to Noise Ratio}
	\acro{SON}{Self-Organizing Network}
	\acro{SPP}{Spatial Poisson Process}
	\acroplural{SPP}[SPPs]{Spatial Poisson Processes}
	\acro{SSS}{Secondary Synchronization Channel}
	\acro{STA}{Standard Tree Algorithm}
        \acro{SAT\(5\)G}{Satellite and Terrestrial Network for \(5\)G}
	\acro{TAS}{Transmit Antenna Selection}
	\acro{TCP}{Transmission Control Protocol}
	\acro{TC}{Transmission Capacity}
	\acro{TDD}{Time Division Duplexing}	
	\acro{TDMA}{Time Division Multiple Access}	
	\acro{TOA}{Time of Arrival}
	\acro{TS}{Terminal Station}
	\acro{TTI}{Transmission Time Interval}
	\acro{TTT}{Time To Trigger}
	\acro{UDM}{Unit Disk Model}
	\acro{UD}{Unit Disk}
	\acro{UE}{User Equipment}
	\acro{ULUTRANSIM}[UL UTRANSim]{R6 Uplink UTRAN Simulator}
	\acro{UL}{Uplink}
	\acro{UML}{Unified Modeling Language}
	\acro{UoI}{User of Interest}
	\acro{UMTS}{Universal Mobile Telecommunications System}
	\acro{URC}{Ultra Reliable Communication}
	\acro{URLLC}{Ultra Reliable Low Latency Communications}
	\acro{WCDMA}{Wideband Code Division Multiple Access}
	\acro{WSN}{Wireless Sensor Network}
	\acro{iid}[\textup{i.i.d.}]{independent and identically distributed}
\end{acronym}

